Orthogonal polynomials on planar cubic curves

Orthogonal polynomials in two variables on cubic curves are considered, including the case of elliptic curves. For an integral with respect to an appropriate weight function defined on a cubic curve, an explicit basis of orthogonal polynomials is constructed in terms of two families of orthogonal polynomials in one variable. We show that these orthogonal polynomials can be used to approximate functions with cubic and square root singularities, and demonstrate their usage for solving differential equations with singular solutions.

==> OPs-on-cubic-curves copy/.git/objects/21/3023d223cd5654d9eca1615c635baf6348cc82 <==
x•ÍJ1"=ÏSôžIº3ù'eñ èm>€$³h&ËLÖç7"x·/ÕTÕÝÜj½tÀ ïú&H"e2RÁ±Í¦"Œ'sÐ.Ö1ûé7Y;pPJ,eŒÚ:ÊÊg‡iaŠ³OÊdÎlþúÅÎ%z,ldVÉ(WJÊçÁ8ôLg"Êo}i¼-"K\áüù%÷ö£O5ò·zmÕ8Փ"¸Wc¦áŽúèþ—œÎ+Ô¸ô‡—K½¥÷gÙ?z»ƒÓ7+m[´

==> OPs-on-cubic-curves copy/.git/objects/66/843906fdb85f05c143ec9ffe92f63fab3a2d5a <==
x•ŽKj1D³Ö)zo­BÈ
ö*Ë©›1X'™'MŽoy'dUð¨*^/cc&f¡àŒ‹£'õX$äôµÁ\¼L¢®´qàSHŽp‰â'µ$ÁI‹sÅ'[Ä:­³{KŠncíœVæ•|_î¼ÁÇޟùU)¿æ^?AÔC4	¨Õ¤ÓoÌî—êÜ
ÿBoPiŸï®päýÚÛÎ0:üܨ©DŽO

==> OPs-on-cubic-curves copy/.git/objects/c9/00e63d2a1673d08d7293b31ec3a58b04dcdc48 <==
xµKjÄ0D³Ö)z?`Zÿ1"UvÉZR+Œ%#Ë¹}´Í²­'z¯bÛ÷2@kù2:3s:("cÑ;åHj)Ë(•]£Íh|F¤ÄAë€à1ÉäUwyύbt°Jú5pL9˜
'A×ØZ‡Oê±}ÐÙj*µÀ«Ã'ÜÞþï×Éý\jë|<~–ï2¶+,±ío jãs
n(ÅLç…Áÿ2.¾ø	©SðœÀû±ÑYNhÆÆPi\PjGoéŠCü¨÷l÷
